Empirical Analysis of Password Reuse and Modification across Online Service

Leaked passwords from data breaches can pose a serious threat to users if the password is reused elsewhere. With more online services getting breached today, there is still a lack of large-scale quantitative understanding of the risks of password reuse across services. In this paper, we analyze a large collection of 28.8 million users and their 61.5 million passwords across 107 services. We find that 38% of the users have reused exactly the same password across different sites, while 20% have modified an existing password to create new ones. In addition, we find that the password modification patterns are highly consistent across different user demographics, indicating a high predictability. To quantify the risk, we build a new training-based guessing algorithm, and show that more than 16 million password pairs can be cracked within just 10 attempts (30% of the modified passwords and all the reused passwords).

==> Makefile <==
# $Id: Makefile,v 1.7 2009/06/20 01:18:01 ale Exp $

LATEX=latex 

BIBTEX=bibtex
BIBFILE=astro.bib
PAPER=pass

TEXFILES = \
	 intro.tex \
	 pass.tex \
	 data.tex \
	 reuse.tex \
	 related.tex \
	 discuss.tex \
	 rule.tex

EPSFIGS = \

EPSGRAPHS = $(wildcard plots/*.eps)

%all:  subdirs $(PAPER).pdf
all: $(PAPER).pdf

subdirs:
	$(MAKE) -C plots

bib:
	$(BIBTEX) pln

%.eps: %.fig
	fig2dev -L eps $< $@
$(PAPER).ps: $(PAPER).dvi
	#dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps
	dvips -P pdf -t letter -o $(PAPER).ps $(PAPER).dvi

$(PAPER).pdf: $(PAPER).dvi
	dvipdf $(PAPER).dvi

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE) 
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf

